Organic Visualization of Document Evolution

Recent availability of data of writing processes at keystroke-granularity has enabled research on the evolution of document writing. A natural step is to develop systems that can actually show this data and make it understandable. Here we propose a data structure that captures a document's fine-grained history and an organic visualization that serves as an interface to it. We evaluate a proof-of-concept implementation of the system through a pilot study with documents written by students at a public university. Our results are promising and reveal facets such as general strategies adopted, local edition density and hierarchical structure of the final text.

==> paper.tex <==
\section{Introduction}\label{introduction}

Writing is an important part of life, and computers have not changed
that fact. On the contrary, they have exacerbated it through social
media \textbf{{[}REF{]}} and text-based communication platforms
\textbf{{[}REF{]}}. Many people's success depend on their writing
skills, including researchers, writers, journalists, \emph{.etc};
however, their success is based on a polished and arguably finished text
document. As stated by Grésillon and Perrin in the Handbook of Writing
and Text Production, ``The written (the product) aims at overcoming the
writing (the process)'' {[}@gresillon2014methodology{]}, which means
that the better the quality of a text, the more work was spent obscuring
and deleting the traces of its own development. However, we don't fully
understand this important, everyday phenomenon, even though the way we
write is tied to how we learn and structure our knowledge
\textbf{{[}REF{]}}. This lack of research is understandable, because the
data that would shed a light on individual writing processes was not
commonly available.

Today, Web services such as Google Drive keep a keystroke-level record
of a document's history. To the extent of our knowledge, the potential
of this information have not been used to make \emph{writing} easier and
more effective, nor to understand the writing process at scale.
Visualizing this data could be the first step toward understanding it,
but, in spite of the vast work on text visualization available
{[}@kucher2015text{]}, visualization research seems to set aside the
near-keystroke granularity. In this aspect, there are two main research
directions. On the one hand, interactive visualizations to analyze text
production are available, but they focus on the finished product. On the
other hand, the systems that aims at the evolution of documents do so at
coarse versioned text. Hence, here we propose an interactive
visualization method in the arguably unexplored field of fine-grained
text production data. Our visualization design follows organic and
ecological approaches to depict the complexity of the writing process,
and to foster exploration of its structure, and its corresponding
evolution through time.

We evaluated our interactive visualization through a case study of
documents written by engineering students in Google Drive. The results
showed that different characteristics of the writing process emerged in
the visualization: general strategies adopted, local edition density,
and in some cases, hierarchical structure of the final text. These
results evoke interesting applications for our proposed system, as it
could be used in several fields, including reviewing, writing, assessing
the depth of knowledge, among other areas. We concluded that the study
and visualization of fine-grained text data enables a deeper
understanding of text, as it augments the finalized product with the
trace of the decisions performed during its evolution.

\section{Background}\label{background}

The field of user interfaces for text visualization is enourmous, with
presence in several areas such as visual text summarization
{[}@hoque2015convisit{]}, topic modeling {[}@sievert2014ldavis{]},
mapping content structure {[}@van2009mapping{]}, recommender systems
{[}@graells2016data{]}, among others (see a survey
{[}@vsilic2010visualization{]}). However, most of these areas focuses on
seemingly \emph{finished} text, \emph{i.e.}, a product of the writing
process of someone (or even something, like a machine), or a corpus of
such products. Instead, our work focuses on the process behind that
generated those documents, particularly in the case of humans: the
\emph{writing} process {[}@gresillon2014methodology{]}. Within this
field there are still different branches that we need to consider. On
the one hand, there is a branch that focuses on making collaborative
writing visible; on the other hand, the branch contains the approaches
that focus at fine-grained, paragraph-length individual writing
strategies.

\textbf{Versioned Text Visualization.} \noindent
In this area, the problem at hand is to understand the structure and
evolution of text accoding to several updates, obtained in versioning
systems (\emph{e.g.}, CVS, SVN, Git, \emph{etc.}). Each update may add
new content, delete prior content, or perform local changes, for
instance, by replacing specific words within a line but mantaining the
context. Currently there are two prominent sources for this kind of
visual interaction: collaborative user-generated content and software
production. The most common data source of collaborative content is
Wikipedia, with tools like History Flow {[}@viegas2004studying{]}, that
visualizes the \emph{revision history} of Wikipedia articles. Such
efforts have appeared also in art installation and visualization
contexts, for instance, through the Notabilia\footnote{http://notabilia.net}
project, which translates there revision histories into collective
deliberation {[}@taraborelli2010beyond{]}. In this aspect, a work
similar to ours in terms of scope is DocuViz {[}@wang2015docuviz{]},
that applied the History Flow approach to collaborative documents in
Google Docs. The other source, software, has generated many projects to
visualize and understand the structure behind the evolution and
collaboration of code , including CVSscan {[}@voinea2005cvsscan{]},
Revision Map {[}@kim2012cumulative{]}, code\_swarm
{[}@ogawa2009code\_swarm{]}, and Software Evolution Storylines
{[}@ogawa2010software{]}. However, in these cases, even though the input
data is text, what matters is the flow structure and control
instructions within the text rather than the textual content itself.

\textbf{Individual Writing Strategies.} \noindent
The individual writing process is important because is tied with
learning and the discover of meaning {[}@zamel1982writing{]}. Thus, it
is relevant to understand these processes. The seminal work of Perrin
{[}@gresillon2014methodology{]} explores how single individuals write in
a short period of time (from 15 to 30 minutes). Caporossi and Leblay
{[}@caporossi2011online{]} showed a graph-based visualization of this
process, where nodes represented text pieces (inserted, deleted); and
edges, their topological and temporal relations.

Our work builds upon graph-based modeling of the writing process
{[}@caporossi2011online{]} to explore Google Docs' fine-grained document
history data, at a level that we denote \emph{keystroke bursts}: coarser
than keystrokes, but much finer than revisions. Our visualization design
draws guidelines from Organic Information Design {[}@fry2000organic{]},
in a way similar to Notabilia, as well as the text visualization
ecological paradigm {[}@wise1999ecological{]} By doing this, we shed a
light on the arguably unexplored field of visualizing individual writing
processes.

\section{System Design}\label{system-design}

The main issue with current state of the art was its foundation in
linear diagrams which failed to deliver the fine-grained complexity of
writing, so we developed an abstract, topological idea of document from
which the data structure derived naturally.

\subsection{Document Operations}\label{document-operations}

First we recognized operations over the document as self-contained units
(the document then passes on to be no more than this chain of atomic
insertions and deletions, like a bead collar). Then, we grouped adjacent
operations according to their linearity (meaning that no voluntary
change in cursor position takes place between any two of them) as in
Perrin's S-notation (2003). This results in coarser insertion and
deletion operations, which we call (linear keystroke) bursts, but also
more coherent and significant units, since a lot of ``indecisions'' and
typographic errors (low-level changes) are eliminated.

Finally, we reordered bursts spatially rather than temporally, as pieces
of a puzzle, joining one to another from the structural points we call
places of insertion (POIs), which are the points between characters and
elements in a document where the blinking cursor can be at.

The graph-like resulting structure is still a fully-working document,
which we formalize in the next section.

\subsection{Data Structure for Text
Evolution}\label{data-structure-for-text-evolution}

The abstract data structure has the form of a directed acyclic graph,
where nodes represent operations, edges are topological relations
between operations and their direction follows the arrow of time. Each
edge points initially to a ``null'' node, meaning a POI. An empty
document in its original state maps to a root node which contains the
time of the file's creation and a single edge which stands for its only
POI. At this point, only an insertion can take place (as a deletion
needs more than one POI), so the next step is the addition of a new
operation node containing the inserted string at the end of the root
edge, from which n+1 edges emerge, where n is the number of characters
inserted, ``opening up'' space with the new places of operation. This
process goes on recursively, always maintaining a tree structure, but
deletions are a different case, since they ``close'' space which can be
at different heights in the hierarchy. A deletion is a node that bundles
together n+1 adjacent edges, where n is the number of characters
deleted, back into a single place of operation. It is easy to see that,
if we delete the whole of what we have written, we'll end up with only
one place of operation left, as in the initial case, though this links
back to the whole graph structure coming from the root node.

\subsection{Design Guidelines}\label{design-guidelines}

Our visualization draws on the ecological (1999) and organic (2000)
approaches to create a natural-looking structure of interdependent
units. This is a departure from the linear, bar chart-style schemas
found on most of current work and aims at a similar change in the
understanding of a document: not as something linear, static, but rather
emergent and dynamic, but also irreversible, meaning that nothing is
really deleted but submerged, in the way of palimpsest.

\subsection{Visual Representation}\label{visual-representation}

As an organic visualization, it is composed of interdependent units, in
this case a glyph that assembles recursively, forming a tree structure.
There is one glyph for each insertion node in the data structure, which
maps to a single insertion node and its first-level out-edges. Deletion
nodes haven't their own glyph but are ``accepted'' by the different
glyphs whose edges it bundles. A glyph is composed by an arc, whose
length represents the POIs created during the linear burst, and a line
which connects it to the burst's POI. When part or the whole of a node
is deleted, the corresponding part of the arc loses opacity and falls
back towards its center. The radius of an arc is doubled each time its
center angle were to surpass \(\Pi\), to avoid arcs from becoming
circles. To avoid spiraling branches, a ``phototropism factor'' was
applied, that mimics plant behavior of growing upwards. Time is
represented using an eight-color palette that mimics seasons, where
nodes are colored according to the session (usually, a day) when they
were inserted.

Our proposed interactive visualization uses glyphs
{[}@ward2008multivariate{]} to represent operations in text.

\begin{figure*}[tb]
\centering
\includegraphics[width=\textwidth]{img/thom-set-up-view.png}
\caption{Experimental set-up (from left to right): the Processing IDE with inspected nodes’ textual content showing in the console; the Processing sketch window with the visualization of the document; a word processor with the highlight tool showing the document.}
\label{fig:exp_setup}
\end{figure*}

\subsection{Design Guidelines}\label{design-guidelines-1}

Here we show a visualization that draws on the organic information
design (2000) and ecological (1999) paradigms to explore Google Docs'
fine-grained document history data\ldots{}

\subsection{Data Structure}\label{data-structure}

The abstract data structure has the form of a directed acyclic graph,
where nodes represent operations, edges are topological relations
between operations and their direction follows the arrow of time. Each
edge points initially to a ``null'' node, meaning a possible place of
operation. An empty document in its original state maps to a node (a

\subsection{Visual Representation}\label{visual-representation-1}

As an organic visualization, it is composed of interdependent units, in
this case a glyph that assembles recursively, forming a tree structure.

This glyph encapsulates a piece of text written ``linearly'', that is,
without a user's voluntary movement to another place in the document.

Time is represented using a color palette that mimics seasons.

\section{Pilot Study}\label{pilot-study}

\begin{figure}[htbp]
\centering
\includegraphics{img/thom-case-studies.png}
\caption{Case studies A, B, C, D and E. Highlight colors were manually
added to show branching structure. \label{fig:case_studies}}
\end{figure}

Our case studies (Figure 2) show that there are three dimensions of the
document that are well captured by the visualization:

\begin{enumerate}
\def\labelenumi{\arabic{enumi}.}
\item
  the amount of work put into it (and in different parts of it); Color
  and general appearance of a branch reveals its amount of work. Case
  studies A, B and C have branches of the same color (meaning they were
  written during one session) whereas D has branches showing many
  appendices of different colors (meaning they were edited in a
  posterior session). This can be recognized intuitively: light-edited
  documents look ``younger'' while heavily-edited ones look ``older''.
\item
  some patterns and strategies adopted by users; Structure of the tree
  reveals the strategies with which the document was written. C, for
  example, shows a very well-defined hierarchical structure, meaning its
  writing bore its final structure in mind from the beginning (typical
  when the assignment stipulates the organization), B shows a draft that
  rewritten and erased (live branches over a dead branch) and D shows
  also the rewriting of a piece of text, only this one was pasted from a
  previous version of the assignment, and also features a lot of editing
  throughout the document.
\item
  the internal organization of the text and its hierarchic structure.
  Branches of a tree mostly correspond to hierarchical structure of the
  text. Branches of A and B match the paragraph division, as they have
  no other hierarchical level. C has a typical hierarchical organization
  (cover information, sections and bibliography) which is perfectly
  matched by the relations of the correspondent branches. D has no more
  structure than paragraph-level as can be intuited by its ``one big
  branch'' appearance.
\end{enumerate}

\section{Discussion}\label{discussion}

We have presented a novel visualization approach for document production
which combines a structural view of the document with an organic visual
scheme, and have showed that it renders visible some complex behavior in
writing. It can be used, for example, to get an overview of the whole of
a document's history in a single image, which is enough to give an idea
of the amount of work put into it and the general strategy adopted:
light vs.~heavily edited documents are intuitively distinguishable and a
text that was rewritten from a draft looks different from one that was
written with a structure in mind. This is something that, for a single
session or single user document and at this level of granularity, none
of the available systems can provide.

With its interactive functions, the system can be used to produce a
segmentation of a document, which in some cases coincides with its
hierarchical structure, but in any case is a naturally occurring
segmentation which follows the thread of thought of the user.

\subsection{Theoretical Implications}\label{theoretical-implications}

Seeing the document as a dynamic structure

\subsection{Practical Implications}\label{practical-implications}

This system could have several uses: as a kind of personality test or
evaluation tool for recruitment in technical environments, for guides to
have a more detailed view on the learning process of their students,
evaluation and, of course, as a real-time writing-aid. Some functions
could even be automatized to show from the data structure, as the
aforementioned segmentation, which can in turn be used to classify
segments according to their need of editing, for example, according to
its relative age on the document.

\subsection{Limitations}\label{limitations}

visualization limitation, external references, multiple users

\subsection{Future Work}\label{future-work}

The visualization shown captures only a subset of the information
contained in the data structure because deletion nodes aren't being
represented as structural elements, the visualization is just a spanning
tree of the whole graph. This leads to the obvious design problem that
the spanning tree is not unique, and so the resulting visualized
structure. Future work will aim at conceiving a way to represent
deletion nodes as structural visual elements. Also, to diminish
occlusion, which currently makes it impossible to analyze larger,
heavily-edited documents, an algorithm for space-awareness will be
implemented for the glyphs.

\subsection{Conclusions}\label{conclusions}

We anticipate this result to provide an integration of computer-aided
writing research by proposing a clear focus on the document as a
well-defined temporal object. Topic segmentation should not be
abstracted from a document's history when possible, and this approach
proves a fair candidate for segmenting a document through its own
writing history.

\clearpage

\section{References}\label{references}

